DataMUX: Data Multiplexing for Neural Networks

In this paper, we introduce data multiplexing (DataMUX), a technique that enables deep neural networks to process multiple inputs simultaneously using a single compact representation. DataMUX demonstrates that neural networks are capable of generating accurate predictions over mixtures of inputs, resulting in increased throughput with minimal extra memory requirements. Our approach uses two key components -- 1) a multiplexing layer that performs a fixed linear transformation to each input before combining them to create a mixed representation of the same size as a single input, which is then processed by the base network, and 2) a demultiplexing layer that converts the base network's output back into independent representations before producing predictions for each input. We show the viability of DataMUX for different architectures (Transformers, and to a lesser extent MLPs and CNNs) across six different tasks spanning sentence classification, named entity recognition and image classification. For instance, DataMUX for Transformers can multiplex up to $20$x/$40$x inputs, achieving $11$x/$18$x increase in throughput with minimal absolute performance drops of $<2\%$ and $<4\%$ respectively on MNLI, a natural language inference task. We also provide a theoretical construction for multiplexing in self-attention networks and analyze the effect of various design elements in DataMUX.

==> _6_diff_arch_runzhe.tex <==
\section{Multiplexing different architectures}
In addition to Transformers, certain special cases for our data multiplexing have been explored for convolutional architectures in the image classification settings for the robustness and data augmentation purpose \cite{rame21, havasi21, soflaei20}.  
The multiplexing in these studies implicitly employed the frontend layers of a convolutional net as nonlinear separation functions, \runzhe{do we still use the term “separation function”?}, and take the superposition. 
The previous work suggested that a convolutional neural network can learn at most 3-4 independent subnetworks concurrently \cite{havasi21}, while with Transformers and linear separation functions, we showed up to 20 inputs can be processed independently without a severe performance drop.
To systematically understand this gap, we test the compatibility of data multiplexing with multilayer perceptrons (MLPs), and convolutional networks (CNNs) on an image classification task.

\subsection{Experimental Setup}

To prevent the distraction from complicated experimental design, we compare the MLP and CNN performance of classifying MNIST digits with different data mixing strategies, as they are the most simple and well-studied models and dataset. We crop each image into 20x20 pixels at the center. Principle component analysis on all 60,000 training images indicates that 86.54\% variance can be explained by top 50 principle components, suggesting that if we only keep the top 50 dimensions for each input image and project them into linearly independent subspaces, ideally we can multiplex 8 inputs as just one input without much information loss. We test the model performances with $N = \{1, 2, 4, 8, 16\}$ multiplexed inputs.

Our MLP consists of a hidden layer with 100 neurons, a demultiplexing layer that maps the 100 hidden neurons to $20\times N$ neurons, and a shared linear readout layer that maps each group of 20 neurons to 10 categories for classification. Our CNN is similar to the classic LeNet \cite{lecun90}, consisting of three convolutional layers with 10 activation maps from 3x3 kernels, 16 activation maps from 4x4 kernels and 120 activation maps from 3x3 kernels, one linear layer maps to 84 hidden neurons, a demultiplexing layer that maps them to $84\times N$ neurons, and a shared linear readout layer that maps each group of 84 neurons to 10 categories for classification. The first two convolutional layers are followed by 2x2 max pooling. Every linear layer or convolution layer in our models is followed by a $\tanh$ activation. Labels are $+1$ for the correct digit and $-1$ for the incorrect digits. And we use the mean squared error (MSE) loss to train all our models.

We train all our models with the standard stochastic gradient decent with fixed learning rates, and the batch size is 32. We also do not apply weight decay or other regularization to the network as many of these design factors can be studied orthogonally to the effect of data multiplexing. 


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{charts/MLPvsCNN-Fig.pdf}
    \caption{average test accuracy for multiplexing MLP and CNN for $N=\{1, 2, 4, 8, 16\}$ inputs on the MNIST classification task. Results are stable cross multiple runs.}
    \label{fig:mlp-vs-cnn}
\end{figure}

\subsection{Multiplexing for MLPs}

The dashed curves in Figure {\ref{fig:mlp-vs-cnn}} show the test performance of MLP with different separation functions for data multiplexing. In the standard setting with only one input, MLP can classify MNIST digits with accuracy at 94.65\%. If we just sum up $N$ input images (separation functions $\phi_i$ are identity mappings), the accuracy decreases quickly in an order of roughly $1/N$ (also lower bound by chance), since the multiplexed inputs are invariant under permutations and MLP must have trouble in distinguishing the right order for predictions. However, after using orthogonal projections uniformly sampled from $\text{SO}(d)$ as separation functions, where $d=400$ is the dimension of input, MLP can easily demultiplex representations and remains 78.27\% average accuracy when $N=8$. Also, similar to Figure \ref{fig:demux_index_results}, the accuracy does not vary much across multiple inputs, with standard derivation at 5\%$\sim$6\% when $N\geq 8$, indicating that the permutation symmetry of inputs is preserved when the network processes information in parallel.

It is worth noting that the random orthogonal projections cannot separate inputs perfectly. Suppose that two linear separation functions $\bm G$ and $\bm H$ are expected to separate all inputs from a manifold $\mathcal M$, we would expect $\bm v^{\top} \bm G^{\top}\bm H\bm u = 0$  for all $\bm v$ and $\bm u \in \mathcal M$. If the dimensionality of the manifold $\mathcal M$ is not too low, then we will need $\bm G^{\top}\bm H = \bm 0$, which implies ${\tt rank}(\bm G) + {\tt rank}(\bm H) \leq d$, but transformations from $\text{SO}(d)$ are full rank. This also means a low-rank transformation which throws away information in advance could help keep zero interference among inputs.

We generate a set of $N$ low-rank orthogonal transformations by dividing $d$ random orthogonal row vectors into $N$ groups, and multiplying them by another $d\times d$ orthogonal matrix. The low-rank separation functions improve the performance compared with $\text{SO}(d)$ when there are many inputs. For small numbers of inputs, its performance is close to $\text{SO}(d)$, which means not much information is lost by compressing inputs with these random low-rank transformations. When $N=8$, its average test accuracy is 83.44\%, which implies information filtered out by the low-rank transformation may grow slower than average interference among different inputs when using random orthogonal projections as $N$ increases. Also, similar to $\text{SO}(d)$, the accuracy also is stable across inputs with std. at about 5\% when $N\geq 8$.

In general, the multiplexing MLPs exhibit similar behavior as multiplexing Transformers. If we normalize accuracy by the number of classes, the relative performance change when $N$ increases follows the same trend as the previous language tasks with enough self-attention heads. This result can be interpreted with a similar theoretical construction in Section \ref{sec:construction}, where ideally each linear layer can process multiplexed input in $N$ linear-independent subspaces.

\subsection{Multiplexing for CNNs}

The solid curves in Figure {\ref{fig:mlp-vs-cnn}} show the test accuracy of multiplexing CNNs as $N$ increases. The vanilla CNN with one input achieves test accuracy at 98.52\%. Similar to MLP, the identity separation function leads to roughly $N$-fold performance drop because of the unidentifiably of input order. The random transformation sampled from $\text{SO}(d)$ makes CNN able to distinguish different inputs. However, its performance is worse than an MLP with the same multiplexing methods. The average accuracy for $\text{SO}(d)$ multiplexing CNN is only 56\% when $N=8$. The performance drop is even across inputs, with std. at about 4\% when $N\geq 8$. Also, note that when there is only one input, the random orthogonal transformation already impairs the performance by 5\% (93.64\%), which is close to the performance of a vanilla MLP with a much smaller capacity. This is because applying $d$-dimensional orthogonal transformation to an image would destroy the spatial locality that CNNs assume. Besides, a series convolutional operation may also make the demultiplexing harder than MLP. 

To make the multiplexing method more compatible with CNNs, we first tried some simple separation functions for images. 2D rotations (\text{SO}(2)) work much better than $\text{SO}(d)$ when $N \leq 2$. When $N=1$, rotating inputs certainly does no harm to the performance. When $N=2$, there is some unavoidable interference between two rotated images, while CNN can still easily distinguish inputs with decent accuracy. However, when $N > 2$, inputs are heavily overlapped, and CNN fails to distinguish many digits. The accuracy among different inputs also varies largely, with std. at 10-24\% when $N\geq 8$, indicating the permutation symmetry of inputs is hard to preserve during optimization. We also tried other simple 2D transformations like mosaic and downsampling so that all inputs are perfectly separated but get blurred. CNN can only answer one of the inputs correctly for this mosaic transformation, since we are only testing the vanilla convolutional architecture, which is not suitable for object detection without proposing bounding boxes.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{charts/CNNkers-Fig.pdf}
    \caption{Averaged test accuracy for multiplexing CNN for $N=\{1, 2, 4, 8, 16\}$ inputs on the MNIST classification task, with different multiplexing strategies. Results are stable cross multiple runs.}
    \label{fig:cnn-kers}
\end{figure}


Figure \ref{fig:cnn-kers} summarizes the performance of other separation functions we used for multiplexing CNN that can preserve spacial locality of images. During multiplexing, we can slide a 3x3 kernel over each input images before summing them up. This make CNN able to distinguish different inputs even with random initialized weights from $\mathcal N(0,1)$ (CNN+Random Kernel). We also make the weights of all $N$ multiplexing kernels learned but the difference is subtle (CNN+Learned Kernel), and the its performance is worse than a multiplexing CNN with 2D rotations. Also, we find that these multiplexing CNN can always answer at most two inputs correctly each time. This is because sliding a small kernel over image is a very constrained linear transformation that cannot do much to separate images, and the permutation symmetry has to be broken during the training dynamics to improve accuracy.

To increase the expressibility of separation functions while keep it compatible with CNN, we apply $N$ small convolutional nets with two layers of 16 3x3 kernels and tanh activation to input images, and sum up their activation maps (CNN+Nonlinear). A multiplexing CNN with this nonlinear separation function is similar to the MIMO approach in the previous study \cite{rame21, havasi21}, and we observe the performance changes consistent with the literature. When $N\leq 4$, its test average test accuracy is above 80\%, which is also better than multiplexing CNN with $\text{SO}(d)$. However, when $N > 4$, the performance drops rapidly. The accuracy across inputs becomes stabler with std. at about 7\% when $N\geq 8$. If we allow higher dimensionally of the multiplexed input than a single input, where the small convolutional nets for multiplexing end with 4 activation maps (CNN+Nonlinear-Expand 4x) or 8 activation maps (CNN+Nonlinear-Expand 8x), we can keep improving the accuracy for larger $N$ while still providing throughput benefit.

Unlike MLP and transformers, our results show that the convolutional structure imposes very strong constraints to data multiplexing. Thus, the maximum number of subnetworks that can be learned simultaneously in a CNN is much less than an MLP, even if the CNN has much more parameters.

==> _experiments_old.tex <==
\section{Experimental setup}
\label{sec:experiments}

To understand the capabilities and limits of data multiplexing for neural networks, we evaluate models with multiplexing on both natural language tasks and vision tasks. For each task, we compare traditional model baselines with models using different multiplexing methods, evaluating on standard performance metrics (e.g. accuracy, F1) and model throughput (instances processed per second).


% \subsection{Natural Language tasks}
For all natural language tasks we use a 12-layer Transformer~\cite{NIPS2017_3f5ee243} based model with a hidden dimension size of 768 built on the Huggingface~\cite{Wolf2019HuggingFacesTS} framework.

\subsection{Retrieval Auxiliary Objective}
Our transformer-based models are all initialized using a model that has been trained using the retrieval task only on the Wikitext-103 dataset~\cite{Merity2017PointerSM} as described in Section~\ref{sec:retrieval_methods}. In addition to initializing all models with retrieval pre-trained weights, we also continue to use the retrieval task as an auxiliary objective during task training, computing the loss as a weighted sum of the task loss and retrieval loss (using $\alpha = 0.1$):
$$
\mathcal{L} = (1-\alpha)\mathcal{L}_{\text{task}} + \alpha\mathcal{L}_{\text{Retrieval}}
$$

\subsection{Token-level classification}
Token-level classification evaluates models' ability to perform token-level tasks on superposed representations. This poses a particular challenge for data-multiplexing models since they must maintain a high-level of individual token disentanglement while also producing representations capable of solving the task. We evaluate token-level classification on the CoNLL-2003 Named Entity Recognition (NER) task~\cite{Sang2003IntroductionTT}.


\subsection{Sentence-level classification}
We evaluate models on a subset of the sentence-level classification tasks found in the General Language Understanding Evaluation (GLUE) benchmark~\cite{wang2019glue}: the sentiment classification task SST-2~\cite{socher2013recursive}, the sentence similarity task QQP~\footnote{\href{https://data.quora.com/First-Quora-Dataset-Release-Question-Pairs}{https://data.quora.com/First-Quora-Dataset-Release-Question-Pairs}}, and the natural language inference tasks MNLI \cite{williams2018broad} and QNLI \cite{wang2019glue, rajpurkar2016squad}. By evaluating on a variety of sentence-level tasks we can gain a better sense of the capabilities of data multiplexing neural networks on tasks that require aggregating sentence representations.

% \subsection{Baselines}
% \begin{enumerate}
%     \item \textbf{12L / 768H Transformer} 

%     % \item Distilled model with Nx smaller hidden size (distilled from teacher): \karthik{This is not a completely fair comparison but I think this will be a strong baseline to add.}
% \end{enumerate}



==> old_results.tex <==
\subsection{Tables}
% sweep on demux architecture; number of hidden layers in the demux block
% demultiplexing strategies
% baseline tables for N =1, 2, 5, 20, 40 --> 2 configurations per N reduction; Layer sweeps 2, 6, 8, 12. 
% lr sweeps 2e-5, 5e-5, 1e-4
% Clean params in scripts; drop last batch fix
% Speed tests
% 

\begin{table*}[t]
\caption{Ablating type of projections for N = 5, conditional prefix }
\label{projections}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{lcccccccccr}
\toprule
Projection & NER &  POS &  SQUAD & SST-2 &   QQP &  QNLI &  MNLI \\
\midrule
Random Gaussian embeddings & & & &  76.9  & 80.02 & 57.82 & 60.47 \\
Random Orthogonal projections & & & &  77.86 & 79.71 & 57.62 & 58.41 \\
Binary encoding & & & & 78.69 & 80.84 & 58.63 & 61.74 \\
Sinusoidal embeddings & & & & 76.67 & 79.3  & 57.42 & 57.65 \\
\midrule
Learnt embeddings (init. with Random Gaussian embeddings) & & & & 61.55 & 79.49 & 54.54 & 40.46 \\
No Projection\\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

\begin{table*}[t]
\caption{Ablating type of projections for N = 20, conditional prefix }
\label{projections}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{lcccccccccr}
\toprule
Projection & NER &  POS &  SQUAD & SST-2 &   QQP &  QNLI &  MNLI \\
\midrule
Random Gaussian Embeddings & & & & 77.71 & 80.08 & 59.43 & 57.25 \\
Random Orthogonal projections & & & &      &       &       &       \\
Binary encoding & & & & 78.96 & 79.41 & 59.62 & 55.69 \\
Sinusoidal embeddings & & & & 78.96 & 79.09 & 60.04 & 54.51 \\
\midrule
Learnt embeddings (init. with Random Gaussian embeddings) & & & & 54.79 & 63.21 & 52.61 & 35.55 \\
No Projection \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

% \begin{table*}[t]
% \caption{Ablating type of projections for N = 5, MLP demuxer }
% \label{projections}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{tabular}{lcccccccccr}
% \toprule
% Projection & NER &  POS &  SQUAD & SST-2 &   QQP &  QNLI &  MNLI \\
% \midrule
% Random Gaussian embeddings \\
% Random Orthogonal projections \\
% Binary encoding \\
% Sinusoidal embeddings \\
% Learnt embeddings (init. with Random Gaussian embeddings) \\
% No Projection \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table*}

\begin{table*}[t]
\caption{Results on GLUE across different number of instances being compressed, conditional prefix demuxer}
\label{projections}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{lcccccccccr}
\toprule
Number of Instances & NER &  POS &  SQUAD & SST-2 &   QQP &  QNLI &  MNLI \\
\midrule
1 & & & & 81.42 & 79.07 & 60.88 & 59.57 \\
2 & & & &  78.81 & 81.65 & 60.79 & 64.02 &  \\
5 & & & & 76.9  & 80.02 & 57.82 & 60.47 &  \\
10 & & & & 78.33 & 79.13 & 59.87 & 57.8  &  \\
20 & & & & 77.71 & 79.94 & 59.43 & 57.25 &  \\
40 & & & & 50.88(nc) & 76.77 & 58.33 & 53.15 & \\ 
100 & & & & nc & nc & nc & nc \\ 
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

% \begin{table}[]
% \begin{tabular}{lllll}
% sst2\_dummy\_parallel\_scratch\_conditional\_2\_mlm\_multisentence\_random\_1.0\_epsilon\_0\_norm\_1\_rc\_1\_lr5e-5  & qqp\_dummy\_parallel\_scratch\_conditional\_2\_mlm\_multisentence\_random\_1.0\_epsilon\_0\_norm\_1\_rc\_1\_lr5e-5  & qnli\_dummy\_parallel\_scratch\_conditional\_2\_mlm\_multisentence\_random\_1.0\_epsilon\_0\_norm\_1\_rc\_1\_lr5e-5  & mnli\_dummy\_parallel\_scratch\_conditional\_2\_mlm\_multisentence\_random\_1.0\_epsilon\_0\_norm\_1\_rc\_1\_lr5e-5  &  \\
% sst2\_dummy\_parallel\_scratch\_conditional\_5\_mlm\_multisentence\_random\_1.0\_epsilon\_0\_norm\_1\_rc\_1\_lr5e-5  & qqp\_dummy\_parallel\_scratch\_conditional\_5\_mlm\_multisentence\_random\_1.0\_epsilon\_0\_norm\_1\_rc\_1\_lr5e-5  & qnli\_dummy\_parallel\_scratch\_conditional\_5\_mlm\_multisentence\_random\_1.0\_epsilon\_0\_norm\_1\_rc\_1\_lr5e-5  & mnli\_dummy\_parallel\_scratch\_conditional\_5\_mlm\_multisentence\_random\_1.0\_epsilon\_0\_norm\_1\_rc\_1\_lr5e-5  &  \\
% sst2\_dummy\_parallel\_scratch\_conditional\_10\_mlm\_multisentence\_random\_1.0\_epsilon\_0\_norm\_1\_rc\_1\_lr5e-5 & qqp\_dummy\_parallel\_scratch\_conditional\_10\_mlm\_multisentence\_random\_1.0\_epsilon\_0\_norm\_1\_rc\_1\_lr5e-5 & qnli\_dummy\_parallel\_scratch\_conditional\_10\_mlm\_multisentence\_random\_1.0\_epsilon\_0\_norm\_1\_rc\_1\_lr5e-5 & mnli\_dummy\_parallel\_scratch\_conditional\_10\_mlm\_multisentence\_random\_1.0\_epsilon\_0\_norm\_1\_rc\_1\_lr5e-5 &  \\
% sst2\_dummy\_parallel\_scratch\_conditional\_20\_mlm\_multisentence\_random\_1.0\_epsilon\_0\_norm\_1\_rc\_1\_lr5e-5 & qqp\_dummy\_parallel\_scratch\_conditional\_20\_mlm\_multisentence\_random\_1.0\_epsilon\_0\_norm\_1\_rc\_1\_lr5e-5 & qnli\_dummy\_parallel\_scratch\_conditional\_20\_mlm\_multisentence\_random\_1.0\_epsilon\_0\_norm\_1\_rc\_1\_lr5e-5 & mnli\_dummy\_parallel\_scratch\_conditional\_20\_mlm\_multisentence\_random\_1.0\_epsilon\_0\_norm\_1\_rc\_1\_lr5e-5 &  \\
% sst2\_dummy\_parallel\_scratch\_conditional\_40\_mlm\_multisentence\_random\_1.0\_epsilon\_0\_norm\_1\_rc\_1\_lr5e-5 & qqp\_dummy\_parallel\_scratch\_conditional\_40\_mlm\_multisentence\_random\_1.0\_epsilon\_0\_norm\_1\_rc\_1\_lr5e-5 & qnli\_dummy\_parallel\_scratch\_conditional\_40\_mlm\_multisentence\_random\_1.0\_epsilon\_0\_norm\_1\_rc\_1\_lr5e-5 & mnli\_dummy\_parallel\_scratch\_conditional\_40\_mlm\_multisentence\_random\_1.0\_epsilon\_0\_norm\_1\_rc\_1\_lr5e-5 & 
% \end{tabular}
% \end{table}

% \begin{table*}[t]
% \caption{Results on GLUE across different number of instances being compressed, MLP demuxer}
% \label{projections}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{tabular}{lcccccccccr}
% \toprule
% Number of Instances & NER &  POS &  SQUAD & SST-2 &   QQP &  QNLI &  MNLI \\
% \midrule
% 1 & & & & \\
% 2 \\
% 5 \\
% 10 \\
% 20 \\ 
% 40 \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table*}

\begin{table*}[t]
\caption{Baselines with smaller models}
\label{projections}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{lcccccccccr}
\toprule
Configuration & Number of parameters & NER &  POS &  SQUAD & SST-2 &   QQP &  QNLI &  MNLI \\
\midrule

2x smaller model & 40942980 (40.94M) & & & & 80.05 & 80.34 & 61.14 & 62.72 &  \\
5x smaller model & 10214016 (10.21M)& & & &  81.88 & 77.99 & 61.67 & 58.36\\
10x smaller model & 4419948 (4.42M)& & & & 81.65 & 77.09 & 60.97 & 56.37 &  \\
20x smaller model & 2022312 (2.02M)& & & & 80.39 & 76.75 & 60.85 & 54.25 &  \\
30x smaller model & 1306620(1.3M) & & & & 80.5  & 76.62 & 61.05 & 50.69 &  \\
\midrule
2 layer model & 53768450(53.76M) & & & & 80.62 & 79.88 & 61.16 & 58.24 \\
4 layer model & 67944194(67.94M) & & & & 81.08 & 80.83 & 61.36 & 62.92 \\
6 layer model & 82119938(82.11M) & & & & 81.31 & 80.58 & 61.34 & 61.71 \\
8 layer model & 96295682(96.29M) & & & & 82.57 & 80.72 & 61.72 & 61.22 \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

\begin{table*}[t]
\caption{Multiplexing with smaller models}
\label{projections}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{lcccccccccr}
\toprule
Configuration & Number of parameters & Number of Instances  & NER &  POS &  SQUAD & SST-2 &   QQP &  QNLI &  MNLI \\
\midrule
10x smaller model & 4419948 (4.42M) & 5 & & & & 78.33 & 77.89 & 56.19 & 53.78 \\
10x smaller model & 4419948 (4.42M) & 10 & & & & 77.98 & 75.93 & 58.25 & 47.49(under optimized) \\
30x smaller model & 1306620(1.3M) & 5 & & & & 74.29 & 74.92 & 58.46 & nc \\
30x smaller model & 1306620(1.3M) & 10 & & & & nc & 74.34 & 56.05 & nc \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

